Accurate Multi-perturbation Localization in Optical Fibers with Polarization-based Forward Sensing

We present a method to accurately localize multiple perturbations from fiber outputs. We cross-correlate received polarizations between two wavelengths, apply peak detection, and interpolate peaks to boost accuracy. We localize five simultaneous perturbations in a 10 GSa/s numerical fiber model with 3.5 m median error.

==> Figures/SOPAS.tex <==
\footnotesize
\pgfplotsset{
    every axis/.style = {
        width = \plotWidth,
        height = \plotHeight,
        font = \footnotesize,
        xticklabel = \empty, 
        yticklabel = \empty,
        scaled x ticks = false,
        scaled y ticks = false,
        xmin = 1700, xmax = 2300,
        ymin = -5000000, ymax = 97000000,
        thick,
        xlabel style = {yshift = .8em},
        ylabel style = {yshift = -.8em}
    }
}

\begin{axis}[
    name = SOPAS1,
    at = {(0, .5\plotSeparation)},
    anchor = south west,
    ylabel = {$a_1[l]$}
]
    % \addplot[\colourOne] table[x = sample_index, y = omega, col sep = comma] {Figures/sopas_1565nm_1pert_sliced.csv};
    \addplot[\colourOne] table[x = sample_index, y = omega, col sep = comma] {Figures/sopas_1565nm_2perts_sliced.csv};

    \coordinate (SOPAS1Peak1) at (1842, 69507633.33210938);
    \coordinate (SOPAS1Peak2) at (2160, 81575826.5487623);
\end{axis}

\begin{axis}[
    name = SOPAS2,
    % xlabel = {$l$},
    at = {(0, -.5\plotSeparation)},
    anchor = north west,
    ylabel = {$a_2[l]$}
]
    % \addplot[\colourTwo] table[x = sample_index, y = omega, col sep = comma] {Figures/sopas_1530nm_1pert_sliced.csv};
    \addplot[\colourTwo] table[x = sample_index, y = omega, col sep = comma] {Figures/sopas_1530nm_2perts_sliced.csv};

    \coordinate (SOPAS2Peak1) at (1809, 69315009.76483032);
    \coordinate (SOPAS2Peak2) at (2103, 82335814.8071946);
\end{axis}

\coordinate (SOPAS2PeakAnchor) at ($(SOPAS2Peak2) + (0, .1)$);
\coordinate (SOPAS1PeakAnchor) at (SOPAS1Peak2 |- SOPAS2PeakAnchor);
\draw[densely dotted, thick] ($(SOPAS1Peak2) + (0, .1)$) -- ($(SOPAS1PeakAnchor) - (0, .1)$);
\draw[densely dotted, thick] ($(SOPAS2Peak2) - (0, .1)$) -- ($(SOPAS2PeakAnchor) + (0, .1)$);
\draw[{Latex[length=.7mm]}-{Latex[length=.7mm]}] (SOPAS1PeakAnchor) -- (SOPAS2PeakAnchor) node[midway] (SOPASPeakDifference) {}; %node[pos = .15, anchor = north] (SOPASPeakDifference) {$t_1 - t_2$};

% \node[rotate = 90, yshift = .25cm] {$a_{1, 2}[l]$};
\node[anchor = north] at (SOPAS1Peak1 |- SOPAS1.south) {$t_1$};
\node[anchor = north] at (SOPAS1Peak2 |- SOPAS1.south) {$t_1$};
\node[anchor = north] at (SOPAS2Peak1 |- SOPAS2.south) {$t_2$};
\node[anchor = north] at (SOPAS2Peak2 |- SOPAS2.south) {$t_2$};

==> Figures/crosscorrelation.tex <==
\footnotesize
\pgfplotsset{
    every axis/.style = {
        width = \plotWidth,
        height = \plotHeight,
        font = \footnotesize,
        xticklabel = \empty, 
        yticklabel = \empty,
        scaled x ticks = false,
        scaled y ticks = false,
        xmin = -1, xmax = 98,
        ymin = -.1, ymax = 1.1,
        thick,
        xlabel style = {yshift = .8em},
        ylabel style = {yshift = -.8em}
    }
}

\begin{axis}[
    name = CrossCorrelation,
    ylabel = {$R[l]$},
    xlabel = {$t_1 - t_2$},
    at = {(0, 0)},
    anchor = west
]
    % \addplot[\colourOne!50!\colourTwo] table[x = lag_index, y = cross_corr_normalized, col sep = comma] {Figures/cross_corr_1pert_sliced.csv};
    \addplot[\colourOne!50!\colourTwo] table[x = lag_index, y = cross_corr_normalized, col sep = comma] {Figures/cross_corr_2perts_sliced.csv};
    \addplot[darkgray] table[x = lag_index, y = threshold, col sep = comma] {Figures/cross_corr_2perts_sliced.csv};
    \coordinate (CorrelationNorthWest) at (axis cs:0,1);
    \coordinate (CorrelationSouthWest) at (axis cs:0,0);
    \coordinate (CorrelationPeak) at (57, 1);
    \draw (52, .914) rectangle (62, 1.05);
    \coordinate (ROISouthWest) at (51, .914);
    \coordinate (ROISouthEast) at (63, .914);
    \coordinate (ROINorthWest) at (51, 1.05);
    \coordinate (ROINorthEast) at (63, 1.05);
\end{axis}

\coordinate (CorrelationPeakAnchor) at (CorrelationPeak |- CrossCorrelation.south);
\draw[dashed, thick] ($(CorrelationPeak) + (0, .1)$) -- (CorrelationPeakAnchor);

==> Figures/crosscorrelation_interpolated.tex <==
\footnotesize

\begin{axis}[
    name = CrossCorrelationInterpolated,
    ylabel = {$R[l]$},
    xlabel = {$t_1 - t_2$},
    at = {(0, 0)},
    anchor = west,
        width = \plotWidth,
        height = \plotHeight,
        font = \footnotesize,
        xticklabel = \empty, 
        yticklabel = \empty,
        scaled x ticks = false,
        scaled y ticks = false,
        xmin = 55, xmax = 59,
        ymin = .9, ymax = 1.05,
        thick,
        xlabel style = {yshift = .8em},
        ylabel style = {yshift = -.8em},
        % legend style = {
        %     at = {(.5, 0)},
        %     anchor = north
        % }
]
    \addplot[\colourOne!50!\colourTwo, only marks, mark = o] table[x = lag_index, y = cross_corr_normalized, col sep = comma] {Figures/cross_corr_2perts_sliced.csv};
    
    \addplot[\colourOne!50!\colourTwo, domain = 55:59] {-138.6498 + 4.914995 * x - 0.04324558 * x * x};
    % \coordinate (CorrelationNorthWest) at (axis cs:0,1);
    % \coordinate (CorrelationSouthWest) at (axis cs:0,0);
    % \coordinate (CorrelationPeak) at (64, 1);
    \coordinate (CorrelationInterpolatedPeak) at (56.826558922, 1.0013264852096);
    % \legend{Sampled, Interpolated}
\end{axis}

% \coordinate (CorrelationPeakAnchor) at (CorrelationPeak |- CrossCorrelation.south);
\draw[dashed, thick] ($(CorrelationInterpolatedPeak) + (0, .1)$) -- (CorrelationInterpolatedPeak |- CrossCorrelationInterpolated.south);

==> Figures/fibre.tex <==
\footnotesize

% Draw fibre input
\node[field, \colourOne] (Input1) {$\lambda_1$};
\node[field, \colourTwo, at = {(Input1.south)}, yshift = -.25cm] (Input2) {$\lambda_2$};

% Draw fibre steps
\coordinate (Fibre1) at ($(Input1.east)!.5!(Input2.east) + (\nodeDistance + \fibreRadius, 0)$);
\coordinate (FibreInput1) at ($(Fibre1) + (0, .33\fibreRadius)$);
\coordinate (FibreInput2) at ($(Fibre1) - (0, .33\fibreRadius)$);
\coordinate (FibreInput1Path) at ($(Input1)!.5!(FibreInput1)$);
\coordinate (FibreInput2Path) at ($(Input2)!.5!(FibreInput2)$);

\draw[draw = none, fill = \fibreEdgeColour] ($(Fibre1) + (0, \fibreRadius)$) -- ++(\sectionCount\sectionLength, 0) arc (90:-90:\fibreRadius) -- ++(-\sectionCount\sectionLength, 0) arc (-90:-270:\fibreRadius);

\draw (Fibre1) circle (\fibreRadius);

\foreach \index [
    evaluate = \index as \indexPlusOne using int(\index + 1)
] in {1,...,\sectionCount}{
    \coordinate[right = \sectionLength of Fibre\index] (Fibre\indexPlusOne);
    \draw ($(Fibre\indexPlusOne) + (0, \fibreRadius)$) arc (90:-90:\fibreRadius);
    \ifthenelse{\index < \sectionCountMinusOne}{
        \node[field, anchor = south] at ($(Fibre\index)!.5!(Fibre\indexPlusOne) + (0, \fibreRadius + .2em)$) {$n = \index$};
    }{}
    \ifthenelse{\index = \sectionCountMinusOne}{
        \node[field] at ($(Fibre\index)!.5!(Fibre\indexPlusOne) + (\fibreRadius, 0)$) {$\cdots$};
    }{}
    \ifthenelse{\index = \sectionCount}{
        \node[field, anchor = south] at ($(Fibre\index)!.5!(Fibre\indexPlusOne) + (0, \fibreRadius + .2em)$) {$n = N$};
    }
}
\draw ($(Fibre1) + (0, \fibreRadius)$) -- ($(Fibre\sectionCountPlusOne) + (0, \fibreRadius)$);
\draw ($(Fibre1) + (0, -\fibreRadius)$) -- ($(Fibre\sectionCountPlusOne) + (0, -\fibreRadius)$);

% Draw EDFA
\node[isosceles triangle, draw, fill = YellowGreen!40!white, at = {(Fibre\sectionCountPlusOne)}, xshift = 1cm, inner sep = 2pt] (EDFA) {EDFA};

% Draw step length
\draw[<->] ($(Fibre1) - (0, \fibreRadius + .35em)$) -- ++(\sectionLength, 0) node[midway, anchor = north] {$L_\textrm{corr}$};

% Draw perturbation
\node[anchor = south, rotate = 180, at = (Fibre\sectionCount)] (Lightning1) {\huge\Lightning};
\node[anchor = west, rotate = 180, at = (Lightning1.east)] (Lightning2) {\huge\Lightning};
\node[at = (Lightning1.north), yshift = -.2em] (Perturbation1) {$D_n[k]$};
\draw[<->] (Fibre1 |- Perturbation1) -- (Perturbation1) node[block, pos = .45, anchor = north, inner sep = 4pt, fill = Yellow!30!white] (PerturbationDistance) {$L - nL_\textrm{corr}$};

% Draw connections
\draw[arrow, thick] (Input1) -| (FibreInput1Path) |- (FibreInput1);
\draw[arrow, thick] (Input2) -| (FibreInput2Path) |- (FibreInput2);
\draw[arrow, thick] ($(Fibre\sectionCountPlusOne) + (\fibreRadius, 0)$) -- (EDFA);
